Illuminating an Ecosystem of Partisan Websites

This paper aims to shed light on alternative news media ecosystems that are believed to have influenced opinions and beliefs by false and/or biased news reporting during the 2016 US Presidential Elections. We examine a large, professionally curated list of 668 hyper-partisan websites and their corresponding Facebook pages, and identify key characteristics that mediate the traffic flow within this ecosystem. We uncover a pattern of new websites being established in the run up to the elections, and abandoned after. Such websites form an ecosystem, creating links from one website to another, and by `liking' each others' Facebook pages. These practices are highly effective in directing user traffic internally within the ecosystem in a highly partisan manner, with right-leaning sites linking to and liking other right-leaning sites and similarly left-leaning sites linking to other sites on the left, thus forming a filter bubble amongst news producers similar to the filter bubble which has been widely observed among consumers of partisan news. Whereas there is activity along both left- and right-leaning sites, right-leaning sites are more evolved, accounting for a disproportionate number of abandoned websites and partisan internal links. We also examine demographic characteristics of consumers of hyper-partisan news and find that some of the more populous demographic groups in the US tend to be consumers of more right-leaning sites.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI


==> sections/Related.tex <==
\section{Related Work}
\label{sec:Related}
Previous studies illuminate various dimensions of the fake news ecosystem. We contextualize our work by providing a brief discussion of key themes in this area. Our work augments previous literature by presenting a data-driven analysis of the producers and consumers of partisan websites, and the traffic forwarding behavior that underpins their sustainability and supports on-line echo chambers. 

% \bano{I have organized related work by their topics. Please revise by: (a) adding an intro line to the beginning of each theme, (b) balance the length of discussions under different theme, (c) remove subjective/verbose comments and report concrete numbers (e.g. surprising results->state the results, other factor->state the factor), (d) since our work adds a new dimension to previous work instead of improving a previous study, there is no needs to super-emphasize the limitations and flaws of previous work: tone down, (e) instead of providing summaries of individual work, focus on ideas and then show how the work contributes to our understanding of the idea via interesting methodology and/or results.}

% \bano{A note about citing other work which applies to the whole paper but especially the Related Work section. Do not directly `address' a citation (e.g. Work like [x] says that what Alice showed in [y] is flawed). Instead, citations should be implicit for example when presenting an idea (the sky is purple[x]), or when quoting a person (Bob said that the sky is purple[y]), or when quoting a bunch of work (an emerging trend is to portray the sky as purple[x,y,z]).}

\mypara{Attitudes towards Partisan news}
Classically political and social science heavily relies on survey-based inferences.
There have been important studies on partisan news media in the US over the past few years. These methods help the community get important insights into the attitudes of audiences towards media \cite{pewSurveyNews3} and the role of social media in news dissemination \cite{pewSurveyNews1}. However, what they lack is an understanding of how the web is shaping these attitudes and trends, and what role social networks play in facilitating spread of partisan information.  
%\newline
A recent work~\cite{Allcot} provides insights into the role of fake news in US elections. The authors use interesting sources of data, such as a crowd-driven website \texttt{Snopes.com} that refutes fake rumors and  conspiracy theories. They further find predictors for believability on face news. Their study
%Albeit being a data-driven study, 
is highly selective towards the fake news phenomenon, 
%More so, their work being `fake news' centric, 
 and ignores the effect of partisan but established news sources on the web and on Facebook such as \textit{Breitbart}, \textit{Infowars}, \textit{ThinkProgress}, \textit{OccupyDemocrats}.
We find in our study that these sources have big enough presence to shape traffic and grab click-through rates as high as 4\% on their posts.
%The implication from the works like~\cite{Allcot} have convinced the computational social science community, that the role of social media and the algorithms that curate content on these platforms is extremely important in understanding phenomena like `Fake News' , `echo chambers' and `filter bubbles'. 
%\newline
Another work\cite{aral2012identifying} suggests that a population that consumes news online has a greater tendency to be polarized than those who do not read online news or consume news through television. 
%These studies highlight that understanding the dynamics of how news media, especially partisan news media, engages users can help in understanding effects like polarization, echo chambers, and filter bubbles. 
% All these works look at the signatures of polarized audiences, but none try to delve deeper into the relation between polar communities and partisan sources of information\ns{Why is this important question?}. More so they fail to explore the connection between the actual news sites and their corresponding social network entities. We try to bridge this gap by looking at correspondence and traffic patterns between the web and social media for partisan sites and the users who engage with them. 

\mypara{Filter bubbles and echo chambers}
Echo chambers refer to the phenomenon when people do not subscribe to views that do not agree with their own. Coupled with recommendation system algorithms, a self-reinforcing ecosystem emerges where users get fed information that suits their opinions\cite{flaxman2016filter}. 
 Analyses of recommendation systems for Facebook users have revealed interesting signals of both the presence of filter bubbles and awareness among some users about their existence~\cite{rader2015understanding}. 
%While the approach of showing users what the algorithm thinks is relevant for user tastes, is good for making people highly engaged, it also raises concerns of creating bubbles of opinions and news that support one's own beliefs.
Recent work~\cite{garimella2017reducing} explores breaking the polarized echo chambers by exposing users to opposing sides of discourse. 
%Despite having interesting user side remedies, there is a missing link between echo chambers and how news sources direct traffic towards each other and towards users. Understanding this side would perhaps give a different angle to this problem.

\mypara{Fake news and social media}
The issue of fake news and conspiracies has received considerable attention since the 2016 US Presidential election. 
%Since then, there has been a considerable push to understand how fake news and conspiracies proliferate and what role do social networks play. 
Various studies~\cite{zannettou2017web,nguyen2012sources,horne2017just,finn2014investigating,kwon2013prominent} have explored the role of social media and platforms like Reddit and 4chan in the process of sharing mainstream and alternative news on the web---but these focus on the lexical value of the language used by fake-news content. 
Starbird et. al~\cite{starbird2017examining} explore the alternative media domain networks by analyzing 58M total tweets related to mass shooting events for a period of about 10 months beginning in January 2016, and provide a qualitative analysis of how alternative news sites propagate and promote false narratives while mainstream media refrains from such behavior. They show the presence of domain clusters that control the flow of information with the alternative news ecosystem and their political polarization. As the scope of this work is limited to the Twitter activity of influential alternative news websites,
%by analyzing suspects through their tweets, it fails to detect and study the entire ecosystem. 
 it does not capture the referrer traffic patterns between social network pages or the actual web pages. Our work augments the findings of this paper using other modalities of data. 



==> sections/notes.tex <==
\section{Facebook section}
1. CDF of number of subscribers and reactions

2. Page linkages analysis 
	 - graph (Fig 9): talk about 2 sides being there; and linkage amongst them. 
     - Do same owner webpages link their Facebook pages (add this analysis to webpage analysis as well).
     
3. Overlap amongst left and right pages (echo chambers)

4. Characterising Facebook page engagement
 How engaging is a Facebook page (how much click through you get per URL using bitly)
 What pages are linked to by embedded urls in the Facebook pages (are these back to the webpages corresponding to the FB page, or is it to other internal websites or other external websites).
 	What do top hubs link to. 
    	Suppose infowars likes breitbart and prisonplanet. Do inforwars links constitute only links to infowars.com, or also to brietbart and prisonplanet or to other external websites. So bar graph with categories: same site, liked sites, internal sites, external sites.
    

\subsection{Bitly analysis}

CDF of number of subscribers,  clicks and reactions






\subsection{misc}
\begin{enumerate}
\item Do embedded URLs in FB pages link back to main website or to other websites as well?
\item Top websites, top hubs and authorities. 
\end{enumerate}

======
Sagar
======

i think the structure and content is reasonable, but we still need to work on abstract and discussion to make an interesting and believable point . Uptill now there are the following take aways : 1) Alexa demographics are very much in line with surveys, 2) Owners of these webpages form cliques 3) the web page upstream links seem to reflect the filter bubble theory as there is a lot of interlinking in the graph with a very high modularity. 4) When we try to mimic the analysis on facebook pages of these web pages, you see extremely high amount of modularity sharply separated by Left and right ideologies 5) From the user side you can see a considerably high probability of overlap among the partisan community than across and more specifically right users tend to follow multiple pages from same partisan groups , compared to left. 

So to stitch all of this together I have 2 thoughts : after Shweta shared the definition of upstream pages, it seems my understanding was wrong, upstream pages do no have specific links but are just pages visited before the current page. So in a way Alexa upstream analysis is also a user behaviour side study, and reflects user stream of visits. Where as the facebook page links are actual liked pages , which require the owner of the page to go and explicitly like it. More over facebook is among the top two upstream sites for almost all partisan sites: this tells me that we are looking at it from the wrong angle, what seems to be is that facebook pages are explicitly making high modularity groups among partisan lines and this is somehow bootstrapping the users of these fb pages to the actual web pages

The second though is we treat the two networks independently and say that this paper proposes a framework to quantify partisan nature of the site based on how deeply embedded is the side on both networks.

========
Shweta
========

To add to Sagar's thoughts- Facebook supports the inter-linkage and spread of the online content of partisan websites by providing an easy medium. Proof to this being the fact that 85% of the 4M Facebook posts are just links. Also, the graph of temporal activity of top left and right Facebook pages points to the fact that the conservative pages were more active on Facebook around the US Election period as compared to liberal ones.
